Broadband ESO/VISIR-Spitzer infrared spectroscopy of the obscured supergiant X-ray Binary IGR J16318-4848

A new class of X-ray binaries has been recently discovered by the high energy observatory, INTEGRAL. It is composed of intrinsically obscured supergiant high mass X-ray binaries, unveiled by means of multi-wavelength X-ray, optical, near- and mid-infrared observations, in particular photometric and spectroscopic observations using ESO facilities. However the fundamental questions about these intriguing sources, namely their formation, evolution, and the nature of their environment, are still unsolved. Among them, IGR J16318-4848 - a compact object orbiting around a supergiant B[e] star - seems to be one of the most extraordinary celestial sources of our Galaxy. We present here new ESO/VLT VISIR mid-infrared (MIR) spectroscopic observations of this source. First, line diagnostics allow us to confirm the presence of absorbing material (dust and cold gas) enshrouding the whole binary system, and to characterise the nature of this material. Second, by fitting broadband near to mid-infrared Spectral Energy Distribution - including ESO NTT/SofI, VLT/VISIR and Spitzer data - with a phenomenological model for sgB[e] stars, we show that the star is surrounded by an irradiated rim heated to a temperature of 3800-5500 K, along with a viscous disk component at an inner temperature of 750 K. VISIR data allow us to exclude the spherical geometry for the dust component. This detailed study will allow us in the future to get better constraints on the formation and evolution of such rare and short-living high mass X-ray binary systems in our Galaxy.

==> symbols.tex <==
\newcommand{\HRule}{\rule{\linewidth}{1mm}}

% USEFUL SYMBOLS

\def\ie{\mbox{\'{\i}}}

% NOMS DE SOURCES

\def\unedzs{1 \mbox{E 1207.4-5209}}
\def\annihilateur{1 \mbox{E 1740.7-2942}}
\def\unedhqu{1 \mbox{E 1841-045}}
\def\qu{\mbox{4U 1630-47}}
\def\azsv{\mbox{A\thinspace} 0620-00}
\def\cicam{\mbox{CI Cam}}
\def\cirxu{\mbox{Circinus X-1}}
\def\cygxu{\mbox{Cygnus X-1}}
\def\cygxt{\mbox{Cygnus X-3}}
\def\grb{\mbox{GRB 990712}}
\def\grojscc{\mbox{GRO J1655-40}}
\def\novmus{\mbox{GRS 1121-68}} %\def\novmus{\mbox{X-ray Nova Muscae 1991}}
\def\novoph{\mbox{GRS 1716-249}} %\def\novoph{\mbox{X-ray Nova Ophiuchi 1993}}
\def\grsdstq{\mbox{GRS 1734-292}}
\def\grsdstn{\mbox{GRS 1739-278}}
\def\grsdsch{\mbox{GRS 1758-258}}
\def\grs{\mbox{GRS 1915+105}}
\def\gx{\mbox{GX 339-4}}
\def\gxtcq{\mbox{GX 354-0}}
\def\igrjstu{\mbox{IGR~J16318$-$4848}}
\def\irasnord{\mbox{IRAS 19124+1106}}
\def\irassud{\mbox{IRAS 19132+1035}}
\def\ksdsvq{\mbox{KS 1724-356}}
\def\ksdstu{\mbox{KS 1731-260}}
\def\lmcxu{\mbox{LMC X-1}}
\def\lmcxt{\mbox{LMC X-3}}
\def\saxjdsqs{\mbox{SAX J1747.0-2853}}
\def\saxjdhzh{\mbox{SAX J1808.4-3658}}
\def\saxjdhdn{\mbox{SAX J1819.3-2525}}
\def\scoxu{\mbox{Sco X-1}}
\def\seyfert{\mbox{Seyfert}}
\def\sgrzcvc{\mbox{SGR 0525-66}}
\def\sgrsvs{\mbox{SGR 1627-41}}
\def\sgr{\mbox{SGR 1806-20}}
\def\sgrdnc{\mbox{SGR 1900+14}}
\def\slx{\mbox{SLX 1735-269}}
\def\smcxu{\mbox{SMC X-1}}
\def\snr{\mbox{SNR G 45.7-0.4}}
\def\ss{\mbox{SS 433}}
\def\swiftjdsct{\mbox{SWIFT J1753.5-0127}}
\def\terzanu{\mbox{Terzan\,\,}1}
\def\vqcqc{\mbox{V404 \mbox{Cyg}}}
\def\vqsqusgr{\mbox{V4641 \mbox{Sgr}}}
\def\wc{\mbox{W 50}}
\def\xtejzqvu{\mbox{XTE J0421+560}}
\def\xtejodh{\mbox{XTE J1118+480}}
\def\xtejqcq{\mbox{XTE J1550-564}}
\def\xtejdsv{\mbox{XTE J1720-318}}
\def\xtejdsqh{\mbox{XTE J1748-288}}
\def\xtejdscc{\mbox{XTE J1755-324}}
\def\xtejdhcn{\mbox{XTE J1859+226}}
\def\xtejdnzh{\mbox{XTE J1908+094}}

% UNITES

\def\angstrom{\mbox{ \scriptsize{A} \vspace*{1.cm}\hspace{-2.9mm}}^{\circ}}
\def\cm{\mbox{ cm}}
\def\cmmoinsdeux{\mbox{ cm}^{-2}}
\def\cmmoinstrois{\mbox{ cm}^{-3}}
\def\cmcube{\mbox{ cm}^{3}}
\def\mdeux{\mbox{ m}^{2}}
\def\mmdeux{\mbox{ mm}^{2}}

\def\arcsecdeux{\mbox{ arc.s}^{2}}
\def\masparan{\times 10^{-3 \, \prime \prime} \mbox{ an}^{-1}}
\def\arcminmoinsdeux{\mbox{arcmin}^{-2}}
\def\rad{\mbox{ rad}}

\def\hz{\mbox{ Hz}}
\def\kg{\mbox{ kg}}
\def\metre{\mbox{ m}}
\def\microns{\mbox{ } \mu \mbox{m}}
\def\msmoinsun{\mbox{ m.s}^{-1}}
\def\msmoinsdeux{\mbox{ m.s}^{-2}}

\def\pc{\mbox{ pc}}
\def\kpc{\mbox{ kpc}}
\def\Mpc{\mbox{ Mpc}}

\def\ms{\mbox{ m\,s}^{-1}}
\def\kms{\mbox{ km\,s}^{-1}}
\def\kmh{\mbox{ km\,h}^{-1}}
\def\Kkms{\mbox{ K\,km\,s}^{-1}}

\def\Mdot{\frac{dM}{dt}}
\def\Msol{\mbox{ }M_{\odot}}
\def\Rsol{\mbox{ }R_{\odot}}
\def\Lsol{\mbox{ }L_{\odot}}
\def\Tsol{\mbox{ }T_{\odot}}
\def\Dsol{\mbox{ }D_{\odot}}
\def\Mstar{\mbox{ }M_{\star}}
\def\Rstar{\mbox{ }R_{\star}}
\def\Lstar{\mbox{ }L_{\star}}
\def\Tstar{\mbox{ }T_{\star}}
\def\Dstar{\mbox{ }D_{\star}}
\def\Mdust{\mbox{ }M_{\rm dust}}
\def\Tdust{\mbox{ }T_{\rm dust}}
\def\Rdust{\mbox{ }R_{\rm dust}}
\def\Porb{P_{orb}}
\def\Pspin{P_{spin}}

\def\mag{\mbox{ magnitude}}
\def\mags{\mbox{ magnitudes}}

\def\mJy{\mbox{ mJy}}
\def\Jy{\mbox{ Jy}}
\def\mJyparbeam{\mbox{ mJy\,beam}^{-1}}
\def\janskyparbeam{\mbox{ Jansky\,faisceau}^{-1}}

\def\keV{\mbox{ keV}}
\def\mT{\mbox{ mT}}

\def\J{\mbox{ J}}
\def\JK{\mbox{ J K}^{-1}}
\def\JKmol{\mbox{ J K}^{-1} \mbox{mol}^{-1}}

\def\K{\mbox{ K}}
\def\degC{^{\circ} \mbox{ C}}

\def\G{\mbox{ G}}

\def\sparan{\mbox{ s an}^{-1}}
\def\paran{\mbox{ an}^{-1}}
\def\jours{\mbox{ jours}}

\def\NAmoinsdeux{\mbox{ N A}^{-2}}
\def\Pa{\mbox{ Pascals}}
\def\Nmmoinsdeux{\mbox{ N m}^{-2}}

\def\W{\mbox{ W}}
\def\WattCmMoinsDeuxMuMoinsUn{\mbox{ W cm}^{-2}\mu \mbox{m}^{-1}}
\def\WMMUM{\mbox{ W m}^{-2}\mu \mbox{m}^{-1}}
\def\Wattmetremoinsdeux{\mbox{ W m}^{-2}}
\def\WparHz{\mbox{ W Hz}^{-1}}
\def\WattmetremoinsdeuxparHz{\mbox{ W m}^{-2}\mbox{ Hz}^{-1}}

\def\erg{\mbox{ erg}}
\def\ergs{\mbox{ erg\,s}^{-1}}
\def\ergcms{\mbox{ erg s}^{-1} \mbox{cm}^{-2}}
\def\ergcmsarcmin{\mbox{ erg cm}^{-2} \mbox{s}^{-1} \mbox{arcmin}^{-2}}
\def\ergcmsang{\mbox{ erg cm}^{-2} \mbox{s}^{-1} \AA}

\def\countss{\mbox{ counts s}^{-1}}
\def\coupss{\mbox{ coups s}^{-1}}

\def\gcmcube{\mbox{ g cm}^{-3}}
\def\gmol{\mbox{ g} \mbox{mol}^{-1}}


% ANGLES

\def\hour{^{h}}
\def\hourp{{\rlap.}^{h}}
\def\min{^{m}}
\def\minp{{\rlap.}^{m}}
\def\sec{^{s}}
\def\secp{{\rlap.}^{s}}

\def\adeg{^{\circ}}
\def\adegp{{\rlap.}^{\circ}}
\def\amin{^\prime}
\def\aminp{{\rlap.}^{\prime}}
\def\asec{^{\prime \prime}}
\def\asecp{{\rlap.}^{\prime \prime}}

% MOLECULES ET TRANSITIONS

%\def\ion[2]{#1$\;${\scshape{#2}}}  % ion, i.e., CII = \ion{C}{ii}
\def\douzecoabb{^{12} \mbox{CO}}
\def\treizecoabb{^{13} \mbox{CO}}
\def\hcoabb{\mbox{H}^{13}\mbox{CO}^{+}}
\def\siodeuxabb{\mbox{SiO}_{2-1}}
\def\siotroisabb{\mbox{SiO}_{3-2}}
\def\siocinqabb{\mbox{SiO}_{5-4}}
\def\csabb{\mbox{CS}}

\def\douzecounzero{^{12} \mbox{CO } (\mbox{J} = 1 - 0)}
\def\douzecodeuxun{^{12} \mbox{CO } (\mbox{J} = 2 - 1)}
\def\treizecodeuxun{^{13} \mbox{CO } (\mbox{J} = 2 - 1)}
\def\treizecounzero{^{13} \mbox{CO } (\mbox{J} = 1 - 0)}
\def\hcoplus{\mbox{H}^{13}\mbox{CO}^{+ }(\mbox{J} = 1 - 0)}
\def\siodeuxun{\mbox{SiO } (\mbox{J} = 2 - 1, v = 0)}
\def\siotroisdeux{\mbox{SiO } (\mbox{J} = 3 - 2, v = 0)}
\def\siocinqquatre{\mbox{SiO } (\mbox{J} = 5 - 4, v = 0)}
\def\csdeuxun{\mbox{CS } (\mbox{J} = 2 - 1)}
\def\hdeux{\mbox{H}_{2}}

\def\Ta{\mbox{T}_{A}^{*}}

% ABBREVATIONS

\def\Al{A_{\rm \lambda}}
\def\Av{A_{\rm V}}
\def\Ak{A_{\rm K}}
%\def\pm{\, \pm \,}
\def\cad{\mbox{c'est-\`a-dire }}
\def\taf{\mbox{tout à fait}}
\def\foot{\footnotemark\footnotetext}
\def\hdeuxromain{\mbox{H\,{\sc ii}}}
\def\nh{N_{\rm H}}
\def\nhone{N_{\rm HI}}
\def\rg{r_{\scriptsize g}}
\def\ltsima{\; \buildrel < \over \sim \;}
\def\simlt{\lower.5ex\hbox{\ltsima}}            % < over MMM
\def\gtsima{\; \buildrel > \over \sim \;}
\def\simgt{\lower.5ex\hbox{\gtsima}}            % > over MMM

% NOMS

\def\M{\mbox{Mirabel}}
\def\R{\mbox{Rodr\'{\i}guez}}
